Hidden Services Protocol for Mixnets

Mix networks (mixnets) provide network-level privacy by routing each communication packet through a sequence of intermediaries, called mixnodes, that randomly delay and cryptographically transform packets before forwarding them, making it difficult for observers to link mixnet entries to exits. While this mechanism protects sender privacy from both external adversaries and the receiver, existing mixnets lack a secure and practical protocol that simultaneously protects receiver (destination) privacy, particularly from the sender. We close this gap. We introduce the first practical and secure hidden-service protocol for mixnets, providing receiver privacy alongside sender anonymity. Our design builds on Single-Use Reply Blocks (SURBs), which enable anonymous replies without revealing the receiver's address. We show, however, that existing approaches to using SURBs expose two practical attacks that can compromise sender or receiver anonymity when the opposing party controls only a single mixnode. We develop defenses against both vulnerabilities. Building on these defenses, we introduce NymHS, a secure and practical hidden-service protocol for mixnets that supports anonymous service discovery, authenticated bidirectional sessions, and asynchronous SURB replenishment. We implement NymHS on the open-source Nym codebase and evaluate its practicality through web-browsing experiments across 118 websites, measuring each of the 27 configurations three times (9,558 page loads). Our results demonstrate that hidden services can be deployed efficiently over mixnets. In particular, increasing the Sphinx payload from 2 KiB to 10 KiB reduces mean page-load latency by approximately 5.2x and decreases communication overhead from 21.7% to 4.3% relative to the current Nym baseline.

==> figures/figure_draft_common.tex <==
% Shared colors/macros for eval workflow figure and step table.
\graphicspath{{figures/icons/}{icons/}}

\definecolor{stepPkcol}{HTML}{D84315}
\definecolor{step1col}{HTML}{1976D2}
\definecolor{step2col}{HTML}{339999}
\definecolor{step3col}{HTML}{228833}
\definecolor{step4col}{HTML}{669922}
\definecolor{step5col}{HTML}{CC7722}
\definecolor{step6col}{HTML}{CC3333}
\definecolor{step7col}{HTML}{994499}
\definecolor{step8col}{HTML}{6633AA}
\definecolor{step9col}{HTML}{00838F}
\definecolor{stepLoadcol}{HTML}{512DA8}
\definecolor{stepMcol}{HTML}{795548}
\definecolor{stepNcol}{HTML}{DD6622}
\definecolor{stepIter310col}{HTML}{8855BB}
\definecolor{stepRep1Ncol}{HTML}{EE8833}

\newcommand{\IterateThreeTenText}{%
  \textcolor{stepIter310col}{Repeat~%
  \textbf{3--10}}%
}


==> figures/figure_draft_table.tex <==
% Step legend (single-column layout; requires figure_draft_common.tex).
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{@{}cl>{\raggedright\arraybackslash}p{0.64\columnwidth}@{}}
  \toprule
  \textbf{Step} & \textbf{Scope} & \textbf{Description} \\
  \midrule
  \textcolor{step1col}{\textbf{1}} & Local & \texttt{POST /metrics/reset} on the CP --- zero counters and start a new epoch \\
  \textcolor{stepPkcol}{\textbf{2}} & Local & Harness directs Playwright to \texttt{GET hs\_pk.sphinx}, the HS recipient key \\
  \textcolor{step2col}{\textbf{3}} & Local & Browser issues one HTTP GET via CP SOCKS (first: document from \texttt{page.goto}; then each referenced CSS, JS, image, \ldots) \\
  \textcolor{step3col}{\textbf{4}} & Mixnet & CP encapsulates one HTTP GET and forwards it through the mixnet \\
  \textcolor{step4col}{\textbf{5}} & Mixnet & Mixnet delivers encrypted request fragments to the HS \\
  \textcolor{step5col}{\textbf{6}} & Origin & HS reassembles fragments and forwards the HTTP GET to the WS \\
  \textcolor{step6col}{\textbf{7}} & Origin & WS returns the HTTP response to the HS \\
  \textcolor{step7col}{\textbf{8}} & Mixnet & HS fragments and encrypts the response, returning it on the client's reply SURBs \\
  \textcolor{step8col}{\textbf{9}} & Mixnet & Mixnet delivers encrypted response fragments to the CP \\
  \textcolor{step9col}{\textbf{10}} & Local & CP reassembles each response and forwards it to the browser \\
  \IterateThreeTenText & Local + Mixnet & As each fetched document is parsed, the browser discovers referenced subresources (e.g., \texttt{index.html} linking an image, a stylesheet, or a script) and issues a separate HTTP GET for each; steps \textbf{3}--\textbf{10} repeat for every such GET until the \emph{load} event \\
  \textcolor{stepLoadcol}{\textbf{11}} & Local & Playwright \texttt{load} event unblocks and reports completion to the harness \\
  \textcolor{stepMcol}{\textbf{M}} & Local & \texttt{GET /metrics} after \emph{load} --- record $T_{\mathrm{load}}$ and counters to CSV \\
  \textcolor{stepNcol}{\textbf{N}} & Local & \texttt{POST /\_\_bench/next} on the WS --- deploy next benchmark template \\
  \textcolor{stepRep1Ncol}{\textbf{1--N}} & Local & \emph{Repeat for each corpus document} until all $118$ templates are visited \\
  \bottomrule
\end{tabular}

